PartDistill: 3D Shape Part Segmentation by Vision-Language Model Distillation

This paper proposes a cross-modal distillation framework, PartDistill, which transfers 2D knowledge from vision-language models (VLMs) to facilitate 3D shape part segmentation. PartDistill addresses three major challenges in this task: the lack of 3D segmentation in invisible or undetected regions in the 2D projections, inconsistent 2D predictions by VLMs, and the lack of knowledge accumulation across different 3D shapes. PartDistill consists of a teacher network that uses a VLM to make 2D predictions and a student network that learns from the 2D predictions while extracting geometrical features from multiple 3D shapes to carry out 3D part segmentation. A bi-directional distillation, including forward and backward distillations, is carried out within the framework, where the former forward distills the 2D predictions to the student network, and the latter improves the quality of the 2D predictions, which subsequently enhances the final 3D segmentation. Moreover, PartDistill can exploit generative models that facilitate effortless 3D shape creation for generating knowledge sources to be distilled. Through extensive experiments, PartDistill boosts the existing methods with substantial margins on widely used ShapeNetPart and PartNetE datasets, by more than 15% and 12% higher mIoU scores, respectively. The code for this work is available at https://github.com/ardianumam/PartDistill.

==> figures/sec4/analysis_view-resolution.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[keepaspectratio, width=0.99\columnwidth]{figures/sec4/analysis_view-resolution.eps}
  \caption{Ablation study about the view numbers and resolutions used in the 2D multiview projection on the ShapeNetPart dataset. 3D mIoU scores are shown, with GLIP being used as the VLM.
  }
  \label{fig:view_resolution}
\end{figure}

==> tables/algorithm.tex <==
\begin{algorithm}
\caption{Will put algorithm block to summarize our whole pipeline}\label{alg:cap}
\begin{algorithmic}
\Require $n \geq 0$
\Ensure $y = x^n$
\State $y \gets 1$
\State $X \gets x$
\State $N \gets n$
\While{$N \neq 0$}
\If{$N$ is even}
    \State $X \gets X \times X$
    \State $N \gets \frac{N}{2}$  
\ElsIf{$N$ is odd}
    \State $y \gets y \times X$
    \State $N \gets N - 1$
\ElsIf{$N$ is odd}
    \State $y \gets y \times X$

\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

==> tables/analysis_projectioninput.tex <==
\begin{table}[ht]
\label{tab:analysis_projectioninput}
\centering
\caption{Analysis on data type used to render multiview images. \vspace{-5px}
}
\resizebox{0.85\columnwidth}{!}{%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{ccccc}
\hline
Shape input   & Texture & Airplane & Chair & Laptop \\ \hline
Mesh          & Y       & xx.x     & xx.x  & xx.x   \\ %\hline
Mesh          & -       &          &       &        \\ %\hline
Dense points  & -       &          &       &        \\ %\hline
Sparse points & -       &          &       &        \\ %\hline
\end{tabular}
}
\end{table}

==> tables/rebuttal/fewshot.tex <==
\begin{table}[]
\centering
\caption{Few-shot segmentation on the PartE dataset (\%mIoU).\vspace{-11px}
}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
Method                & Bottle & Cart& Chair& \multicolumn{1}{l}{Display } & \multicolumn{1}{l}{Kettle} & \multicolumn{1}{l}{Knife} & \multicolumn{1}{l}{Overall} \\ \hline
\makecell{Baseline} & 72.4& 74.5& 83.4& 74.3& 64.3& 68.0& 56.4\\ \hline
Ours                  & \textbf{84.6}&\textbf{90.1}  & \textbf{88.4}& \textbf{87.4}& \textbf{78.6}& \textbf{71.4}& \textbf{65.9}                        \\ \hline
\end{tabular}
}
\vspace{-19px}
\end{table}

==> tables/rebuttal/openscene.tex <==
\begin{table}[]
\centering
\caption{Zero-shot seg. on the ShapeNetPart dataset (\%mIoU)*.\vspace{-9px}
}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
Method                & Airplane & Bag & Cap & \multicolumn{1}{l}{Chair} & \multicolumn{1}{l}{Earphone} & \multicolumn{1}{l}{Guitar} & \multicolumn{1}{l}{Overall} \\ \hline
\makecell{OpenScene~[A]} & 34.4& 63.8& 56.1& 59.8& 62.6& 69.3& 52.9\\ \hline
Ours                  & \textbf{40.6}& \textbf{75.6}& \textbf{67.2}& \textbf{65.0}& \textbf{66.3}& \textbf{85.8}& \textbf{63.9}\\ \hline
\end{tabular}
}

\resizebox{0.85\columnwidth}{!}{
{\tiny \hskip-13px*For fairness, we use the same VLM (CLIP~[34]) and the same 3D backbone (PointM2AE~[44]) \par}}
\vspace{-17px}
\end{table}
